Addressing "Documentation Debt" in Machine Learning Research: A Retrospective Datasheet for BookCorpus

Recent literature has underscored the importance of dataset documentation work for machine learning, and part of this work involves addressing "documentation debt" for datasets that have been used widely but documented sparsely. This paper aims to help address documentation debt for BookCorpus, a popular text dataset for training large language models. Notably, researchers have used BookCorpus to train OpenAI's GPT-N models and Google's BERT models, even though little to no documentation exists about the dataset's motivation, composition, collection process, etc. We offer a preliminary datasheet that provides key context and information about BookCorpus, highlighting several notable deficiencies. In particular, we find evidence that (1) BookCorpus likely violates copyright restrictions for many books, (2) BookCorpus contains thousands of duplicated books, and (3) BookCorpus exhibits significant skews in genre representation. We also find hints of other potential deficiencies that call for future research, including problematic content, potential skews in religious representation, and lopsided author contributions. While more work remains, this initial effort to provide a datasheet for BookCorpus adds to growing literature that urges more careful and systematic documentation for machine learning datasets.

==> tables/datacard2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\begin{small}
\def\arraystretch{1.25}%
\begin{tabular}{|l|l|l|}
\hline
\textbf{Meta-attribute}                    & \textbf{Attribute}       & \textbf{Information}                       \\ \hline
\multirow{3}{*}{Motivation}                & Original Use Case        & Sentence embedding                         \\ \cline{2-3} 
                                           & Original Authors         & Zhu and Kiros et al. \cite{zhu2015aligning}                                        \\ \cline{2-3} 
                                           & Original Funding         & Google, Samsung, NSERC, CIFAR, ONR                               \\ \hline
\multirow{6}{*}{Composition}               & Total Instances          & 11,038 books                                    \\ \cline{2-3} 
                                           & Unique Instances         & $\leq$7,185 books                                     \\ \cline{2-3} 
                                           & Sample or Complete                  & Sample ($\approx$2\% of Smashwords as of 2014)                                       \\ \cline{2-3} 
                                           & Missing Data             & 98 empty book files, $\leq$655 truncated files                                 \\ \cline{2-3} 
                                           & Noise and Redundancies   & Duplicate books and sentences, preamble text       \\ \cline{2-3} 
                                           & Sensitive Information    & Personal contact details (e.g. author emails)              \\ \hline
\multirow{4}{*}{Collection}                & Collection Mechanism     & Web scraping                                   \\ \cline{2-3} 
                                           & Sampling Strategy        & Convenience                                \\ \cline{2-3} 
                                           & Ethical Review          & None stated                                \\ \cline{2-3} 
                                           & Author Consent          & None                                       \\ \hline
\multirow{3}{*}{Cleaning and Labeling}     & Cleaning Done           & None stated, some implicit                                        \\ \cline{2-3} 
                                           & Labeling Done           & None stated (genres labeled by Smashwords)                                        \\ \cline{2-3} 
                                           & Software Used            & Not specified                                    \\ \hline
\multirow{2}{*}{Uses}                      & Original Use Case        & Sentence embedding                         \\ \cline{2-3} 
                                           & Other Notable Uses       & Language models (e.g. GPT \cite{radford2019language}, BERT \cite{devlin2018bert})       \\ \hline
\multirow{4}{*}{Distribution}              & Original Distribution    & Author website                             \\ \cline{2-3} 
                                           & Replicate Distribution     & Available as BookCorpusOpen \cite{bookcorpusopencard}                \\ \cline{2-3} 
                                           & Copyright/Terms of Use   & None                                       \\ \cline{2-3} 
                                           & Third Party Restrictions & None                                       \\ \hline
\multirow{4}{*}{Maintenance and Evolution} & Original Maintainers     & None (formerly Zhu and Kiros et al. \cite{zhu2015aligning})                                 \\ \cline{2-3} 
                                           & Replicate Maintainers & Shawn Presser collected BookCorpusOpen \cite{bookcorpusopencard}                        \\ \cline{2-3} 
                                           & Corrections or Erratum                    & None                                 \\ \cline{2-3} 
                                           & Methods to Extend             & ``Homemade BookCorpus'' software \cite{soskkobayashi2018bookcorpus}                                 \\ \hline

\end{tabular}
\end{small}
\caption{Summary ``Data Card'' for BookCorpus. Detailed information about each attribute is in the datasheet.}
\end{table}
